Data-driven Protection of Transformers, Phase Angle Regulators, and Transmission Lines in Interconnected Power Systems

This dissertation highlights the growing interest in and adoption of machine learning (ML) approaches for fault detection in modern power grids. Once a fault has occurred, it must be identified quickly and preventative steps must be taken to remove or insulate it. As a result, detecting, locating, and classifying faults early and accurately can improve safety and dependability while reducing downtime and hardware damage. ML-based solutions and tools to carry out effective data processing and analysis to aid power system operations and decision-making are becoming preeminent with better system condition awareness and data availability. Power transformers, Phase Shift Transformers or Phase Angle Regulators, and transmission lines are critical components in power systems, and ensuring their safety is a primary issue. Differential relays are commonly employed to protect transformers, whereas distance relays are utilized to protect transmission lines. Magnetizing inrush, overexcitation, and current transformer saturation make transformer protection a challenge. Furthermore, non-standard phase shift, series core saturation, low turn-to-turn, and turn-to-ground fault currents are non-traditional problems associated with Phase Angle Regulators. Faults during symmetrical power swings and unstable power swings may cause mal-operation of distance relays and unintentional and uncontrolled islanding. The distance relays also mal-operate for transmission lines connected to type-3 wind farms. The conventional protection techniques would no longer be adequate to address the above challenges due to limitations in handling and analyzing massive amounts of data, limited generalizability, incapability to model non-linear systems, etc. These limitations of differential and distance protection methods bring forward the motivation of using ML in addressing various protection challenges.

==> Vita_pkb.tex <==
%%%% This section describes the curriculum vitae 
%%% Education
%%% Professional Experience
%%% Publications
%%% Works in review or in preparation for submission
\chapter*{\centering {Curriculum Vitae}}
\vspace{-1cm}
Name of Author: Pallav Kumar Bera

Place of Birth: West Bengal, India

Major: Electrical Engineering

\begin{noindent}
\Large{\textbf{Education:}}
\end{noindent}
\begin{itemize}
    \item
Ph.D., August 2021, Syracuse University, Syracuse, USA (Expected)
\item
M.Tech., Indian Institute of Technology, Roorkee, India, 2014
\item
B.Tech., Haldia Institute of Technology, West Bengal, India, 2011

\end{itemize}
\begin{noindent}
\Large{\textbf{Professional Experience:}}
\end{noindent}

\begin{itemize}
\item Graduate Assistant, Department of Electrical Engineering and Computer Science, Syracuse University, Syracuse, USA, August 2016- Aug 2021.
\item Teaching Professor, Electrical Engineering Dept., Kalinga Institute of Industrial Technology, India, July 2014 – Aug 2016.
\item Teaching Assistant, Electrical Engineering Dept., Indian Institute of Technology, Roorkee, India,  July 2013- June 2014.

\end{itemize}

\begin{noindent}
\Large{\textbf{Published Papers:}}
\end{noindent}

\begin{itemize}
     \item P. K. Bera, and C. Isik (May, 2021). “A Data Mining based Protection and Classification of Transients for Two-Core Symmetric Phase Angle Regulators”. In: IEEE Access. 
     
    \item P. K. Bera, C. Isik, and V. Kumar (July, 2020). “Discrimination of Internal Faults and Other Transients in an Interconnected System with Power Transformers and Phase Angle Regulators”. In: IEEE Systems Journal.
    
    \item P. K. Bera, C. Isik and V. Kumar  (April 1-2, 2021). ``Distance Protection of Transmission Lines Connected to Type-3 Wind Farms". In: Annual IEEE Power and Energy Conference (PECI), Illinois, USA.
 
    \item P. K. Bera, C. Isik (April 7-9, 2021). ``Identification of Stable and Unstable Power Swings using Pattern Recognition". In: 13th Annual IEEE Green Technologies Conference (GreenTech), USA.

   
     \item S. R. Pani, P. K. Bera and V. Kumar (Dec. 2020) ``Detection and Classification of Internal Faults in Power Transformers using Tree based Classifiers". In: IEEE International Conference on Power Electronics, Drives and Energy Systems (PEDES), India, 2020.
     
    \item P. K. Bera, R. Kumar, and C. Isik (Dec. 2018). “Identification of internal faults in indirect symmetrical phase shift transformers using ensemble learning”. In: 2018 IEEE International Symposium on Signal Processing and Information Technology (ISSPIT), Louisville, KY, USA.
    
     \item {S. K. Bhasker, P. K. Bera, V. Kumar and M. Tripathy (Dec. 2015) ``Differential Protection of Indirect Symmetrical Phase Shift Transformer using Wavelet Transform". In: Annual IEEE India Conference (INDICON), New Delhi, India.}
     
    \item {S. K. Bhasker, P. K. Bera, V. Kumar and M. Tripathy (Nov. 2015) ``Differential Protection of Indirect Symmetrical Phase Shift Transformer and Internal Faults Classification using Wavelet and ANN". In: IEEE Region 10 Conference (TENCON), Macao, China.}
    
\end{itemize}

% [1]  \textbf{W.  P.  Jean  Philippe},  S.  Eftekharnejad,  and  P.  K.  Ghosh,  “Development of a new voltage stability index and its implementation considering voltage measurement uncertainty,” IET Generation, Transmission \& Distribution, 2019.

% [2]  \textbf{W.  P.  Jean  Philippe},  S.  Eftekharnejad,  and  P.  K.  Ghosh,  “A  copula-based uncertainty modeling of wind power generation for probabilistic power flow study,” in 2019 the 7th International Conference on Smart Energy Grid Engineering (SEGE). IEEE, 2019, pp. 218–222.

% [3]  \textbf{W. P. Jean Philippe}, E. Iannone, S. Eftekharnejad, and P. K. Ghosh, “Selection of conventional generation resources for optimal replacement by wind power generations,” in 2020 Texas Power and Energy Conference (TPEC). IEEE, 2020, pp. –.

% [4]  \textbf{W. P. Jean   Philippe}, M. Hashemi, Y. Zhou, B. Ansumana, and S. Eftekharnejad, “Supplementing spinning reserves with demand response under wind generation uncertainty,” in 2020 IEEE PES Innovative Smart Grid Technologies Conference. IEEE, 2020, pp. –.


%  [5] R. Ma, S. Jin, S. Eftekharnejad, R. Zafarani, and \textbf{W.P. Jean Philippe}, "A Probabilistic Cascading Failure Model for Dynamic Operating Conditions", IEEE Access, 2020.
% \vspace{1cm}

% \begin{noindent}
% \Large{\textbf{Working Papers:}}
% \end{noindent}

% \begin{itemize}
%     \item \textbf{W. P. Jean Philippe}, S. Zhang, S. Eftekharnejad, P. K. Ghosh and P. K. Varshney, “Uncertainty Modeling of Wind Farm Production for Power System Operational Planning Studies,” in preparation for submission.
    
%     \item \textbf{W. P. Jean Philippe}, S. Eftekharnejad, and P. K. Ghosh, “Impact of bivariate copula selection on scheduling of spinning reserves under high wind power penetration,” in preparation for submission.
    
%     \item \textbf{W. P. Jean Philippe}, S. Eftekharnejad, and P. K. Ghosh, “Optimal Replacement of Conventional Synchronous Generators by Wind Power Generations,” in preparation for submission.
    
   
    
     %\item M. Hashemi, \textbf{W .P. Jean Philippe}, and S. Eftekharnejad, "Investigating the Feasibility of Deploying Community-based Solar Generation for Power System Expansion Planning", in preparation for submission.
    
    
% \end{itemize}







==> abs.tex <==
\begin{center}
    \LARGE{\textbf{Abstract}}
\end{center}
This study demonstrates the increasing interest and rapid expansion in the use of machine
learning techniques to successfully address the technical challenges of the smart grid from various aspects. It is
also revealed that some issues still remain open and worth further research efforts, such as the high-performance
data processing and analysis for intelligent decision-making in large-scale complex multi-energy systems,
lightweight machine learning-based solutions, and so forth.

Machine learning will
be one of the major drivers of future smart electric power systems,
Such significantly improved system condition awareness and data
availability demands for machine learning-based solutions and tools to
carry out efficient data processing and analysis to promote the system
operational management and decision-making.

It is widely agreed that the conventional computational and
management techniques being used in power systems are no longer
adequate in addressing the aforementioned issues due to their limitations
in handling and analyzing the massive amount of data, limited
generalizability of conventional models, the inadequacy of autonomous
operations and real-time processing, high dependence on centralized
control strategies, lack of the capability to model highly non-linear
systems, and so forth. The inadequacy and limitations of conventional
computational techniques bring forward the motivation of using machine
learning techniques in addressing various smart grid challenges.

In the past decade, the electrical power systems have been undergoing
a transition from the conventional energy systems to a more efficient
next-generation smart grid system.
The integration and incorporation of IoT devices into
the grid infrastructure is a prime step towards the future smart grid.
The IoT integration
in the smart grid brings about additional challenges to the
management of smart grids, e.g., the timely delivery of critical operational
information, the efficient process of the vast amount of field data,
and cyberspace security issues. These challenges need to be appropriately
addressed through the use of advanced technologies, e.g., the
phasor measurement unit placement, advanced analytical tools, and
machine learning-based solutions.
The integration of various DGs introduces numerous challenges, e.g.,
load forecast [8,9], fault and failure analysis [10], demand-side management
[11], non-intrusive load monitoring (NILM) [12], cyberspace
security [13], electricity theft detection [14], and islanding detection
[15] among others.

cyberspace security in [4],
electric load forecasting [16], demand response [17], and fault and
failure detection and diagnosis [18],


The integration of advanced information and
communication technologies, in particular IoT, in the power grid infrastructure
is one of the primary steps towards the smart grid



predictions
of load and price [37], cascading failure prediction [38], power
generation and control [39], fault detection and diagnosis [41,40],
DSM [42], and detection of cyberspace attacks


Since the conventional power grid is
under a transformation to a more efficient and reliable smart grid, this
transition puts forward increased stress on the century-old power grid
infrastructure for further investment to ensure safe and reliable energy
supply to the consumers. Therefore, efficient and intelligent mechanisms
for fault and failure detection and diagnosis must be formulated.





%%%Completely Done
With the increasing penetration of renewable energy resources and
electronic devices, the scale and complexity of the power system is
growing in all sectors, e.g., generation, transmission, distribution systems.
Once
the fault occurs, it is required to timely identify and perform a wide
range of protective measures to clear or insulate it. Hence, an early and
accurate detection, location and classification of faults can increase
safety and reliability and reduce downtime and interruption time.


the modern power
system is currently challenged by the growing volumes of data of various
nature, the urging need of data storage, the ever-increasing penetration
of distributed generations and technological advancements. There is no
doubt that the modern power system calls for a more reliable and flexible
power system protection and control. Therefore, a huge number of
monitoring devices (e.g., advanced metering infrastructure, AMI, supervisor
control and data acquisition networks, SCADA, wide area
measurement system, WAMS), capable of exchanging information are
connected to their respective networks for guaranteeing the system
operation (Ibrahim et al., 2020). These data tend to be heterogeneous,
multi-modal, decentralized, and highly nonlinear, imposing significant
challenges to conventional model-driven methods. Inevitably, those
conventional techniques used in power systems are no longer adequate
in dealing with the aforementioned issues because of their limitations in
analyzing the generalizability of conventional models, storing the large
volume of data, the adequacy and efficiency of real-time processing.

Data-driven methods designed for acquiring hidden knowledge from
empirical data gradually attract the researchers’ interest, where machine
learning techniques provides a promising way to meet the challenges
brought by big data.


\hspace{8mm}To ensure the continuous operation of reliable and economically efficient power systems, system operators and planners need to study the impact of WPGs on bulk power systems and determine the best ways to manage their variability. Such studies require efficient and effective probabilistic models characterizing the variable nature of wind power. Therefore, this dissertation develops new methodologies for modeling the uncertainty and variability of WPG. The developed methods are combined with stability indices to form analytical tools for analyzing the impact of increased penetration of wind energy on power system steady-state stability. The case study results show that the developed methods simulate real-world wind power scenarios, which lead to an accurate assessment of the impact of wind generation uncertainty on power systems. 




\hspace{8mm} With large-scale adoption of renewable energy, a significant amount of conventional generation units could be replaced with wind energy resources. The best way to use the variable WPG and the remaining conventional generation resources, for continuous balance between load and generation, remains to be determined. Within this context, this dissertation investigates the problem of optimal substitution of conventional generation units by wind-powered generators, while considering the variability of WPG and the uncertainties of energy demand. The goal is to ensure that during unplanned wind power unavailability, the system has the ability to meet the load demand, and maintain steady acceptable voltage levels in the grid. A two-stage solution methodology is proposed to the problem in consideration. The first stage determines the best candidates, among conventional generator (CG) resources, for retirement and replacement by WPG resources. The best candidates for wind replacement are selected such that the adverse impacts of wind power intermittency on system stability and reliability are minimized. In the second stage, the expected amount of wind generation to be added at each retired CG bus is determined. The simulation results show that the developed method facilitates the integration of high wind energy with a reduced need for additional spinning reserves in the system.



==> glossary.tex <==
%%%% Glossary for term used and defined in the thesis
\chapter*{Glossary}
%\addcontentsline{toc}{chapter}{Glossary}



